Adaptive test for ergodic diffusions plus noise

We propose some parametric tests for ergodic diffusion-plus-noise model, which is a version of state-space modelling in statistics for stochastic diffusion equations. The test statistics are classified into three types: likelihood-ratio-type test statistic; Wald-type one; and Rao-type one. All the test statistics are constructed with quasi-likelihood-functions for local mean sequence of noised observation. We also simulate the behaviour of them for several practical hypothesis tests and check the convergence in law of test statistics under null hypotheses and consistency of the test under alternative ones. We apply the method for real data analysis of wind data, and examine some sets of the hypotheses mainly with respect to the structure of diffusion coefficient.

==> preamble.tex <==
\usepackage[a4paper,top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% maketitle
\usepackage[UKenglish]{babel}
\usepackage{authblk}

% math fonts and symbols
\usepackage{amsfonts,amsmath,amsthm,amssymb} % \text and \mathbb command
\usepackage{mathrsfs} % script type font
\usepackage{stmaryrd} % new bracket

% Bernoulli Journal
\RequirePackage[OT1]{fontenc}
\usepackage[square,numbers]{natbib}
%\bibliographystyle{abbrvnat}
\bibliographystyle{apalike}

\RequirePackage[allcolors=black]{hyperref}

% others
\usepackage{comment} % commenting out multiple lines
\usepackage{graphicx} % graphics
\usepackage{setspace}
\usepackage{subcaption}

\allowdisplaybreaks[1]
%\setlength\parindent{15pt}

